What do CNNs Learn in the First Layer and Why? A Linear Systems Perspective

It has previously been reported that the representation that is learned in the first layer of deep Convolutional Neural Networks (CNNs) is highly consistent across initializations and architectures. In this work, we quantify this consistency by considering the first layer as a filter bank and measuring its energy distribution. We find that the energy distribution is very different from that of the initial weights and is remarkably consistent across random initializations, datasets, architectures and even when the CNNs are trained with random labels. In order to explain this consistency, we derive an analytical formula for the energy profile of linear CNNs and show that this profile is mostly dictated by the second order statistics of image patches in the training set and it will approach a whitening transformation when the number of iterations goes to infinity. Finally, we show that this formula for linear CNNs also gives an excellent fit for the energy profiles learned by commonly used nonlinear CNNs such as ResNet and VGG, and that the first layer of these CNNs indeed perform approximate whitening of their inputs.

==> correlations.tex <==
% RANDOMMMMM
% labels : ['True' 'Random']
% random_labels : [0. 1.]
% 50990it [02:03, 412.96it/s]
%       model_name  correlation    power  labels
% 4529         vgg     0.210081    74300    True
% 8153         vgg    -0.034576  4999900  Random
% 9059         vgg     0.324996  2632700    True
% 10871        vgg     0.124185  2349900    True
% 14495        vgg     0.093174  4999900  Random
% 16307        vgg    -0.080519   951000  Random

% 50990it [03:10, 267.58it/s]
%       model_name  correlation    power  labels
% 905       resnet     0.900715   650200    True
% 1811      resnet     0.931074  1207000  Random
% 2717      resnet     0.914886   277000  Random
% 3623      resnet     0.934138   613200    True
% 4529      resnet     0.947693  1049200  Random
% 5435      resnet     0.904511   485800    True
% 6341         vgg     0.953092   913800    True
% 7247         vgg     0.966298   826100  Random
% 10871        vgg     0.957227   769600    True
% 12683        vgg     0.969127   888300  Random
% 18119        vgg     0.958729  1055400  Random
% 19931        vgg     0.966898  1004200    True
%       model_name  correlation    power  labels
% 4529         vgg     0.943618  1290700    True
% 9059         vgg     0.960101  1336300    True
% 10871        vgg     0.936561  1327900    True
% IMAGENET
%          model_name  correlation   power
% 3   resnext50_32x4d     0.899693  932850
% 5     squeezenet1_0     0.895959  751600
% 6          resnet18     0.919250  668200
% 7       densenet121     0.902554  766900
% 8         googlenet     0.896628  674150
% 57         random_7     0.114263  500000
% ####################3
% car_vs_truck
%       model_name  correlation  power
% 12797   vgg11_bn     0.923609    116
% 15797   vgg11_bn     0.941005    120
% 17797   vgg11_bn     0.924145    145
% ####################3
% dog_vs_frog False False
% random_labels : [0. 1.]
% seed : [5.091123e+06 8.560000e+02 3.901200e+04]
% iteration : [1. 2. 3.]
% labels : ['true' 'random']
% 50990it [01:22, 621.67it/s]
% ####################3
% dog_vs_frog
%      model_name  correlation  power
% 797    vgg11_bn     0.888124    202
% 2797   vgg11_bn     0.921910    166
% 3797   vgg11_bn     0.912551    318
% ####################3
% dog_vs_cat False False
% random_labels : [0. 1.]
% seed : [3.901200e+04 5.091123e+06 8.560000e+02]
% iteration : [1. 2. 3.]
% labels : ['true' 'random']
% 50990it [01:21, 623.25it/s]
% ####################3
% dog_vs_cat
%       model_name  correlation  power
% 18797   vgg11_bn     0.954198    252
% 21797   vgg11_bn     0.960982    266
% 22797   vgg11_bn     0.936362    257
% ####################3
% bird_vs_plane False False
% random_labels : [0. 1.]
% seed : [3.901200e+04 5.091123e+06 8.560000e+02]
% iteration : [1. 2. 3.]
% labels : ['true' 'random']
% 50990it [01:21, 624.07it/s]
% ####################3
% bird_vs_plane
%       model_name  correlation  power
% 24797   vgg11_bn     0.962885    150
% 27797   vgg11_bn     0.967227    147
% 29797   vgg11_bn     0.956020    155
% ####################3
% boat_vs_plane False False
% random_labels : [0. 1.]
% seed : [3.901200e+04 5.091123e+06 8.560000e+02]
% iteration : [1. 2. 3.]
% labels : ['true' 'random']
% 50990it [01:22, 620.77it/s]
% ####################3
% boat_vs_plane
%       model_name  correlation  power
% 6797    vgg11_bn     0.954053    169
% 9797    vgg11_bn     0.947894    198
% 11797   vgg11_bn     0.971044    217










% \begin{figure*}[t!]%%
%   \vskip 0.2in
%   \centering
%   \subfloat[\centering PCA Component 2 ($0.63\pm 0.02$)]{{\label{trueradomenergy}\includegraphics[width=0.32\linewidth]{figures/component_labeling/split_data_original_dataset_component_for_labelization_0.0__comparing labels just energy.pdf} }}%
%   \hfill
%   \subfloat[\centering PCA Component 4 ($0.77\pm 0.01$)]{{\label{trueradomenergy}\includegraphics[width=0.32\linewidth]{figures/component_labeling/split_data_original_dataset_component_for_labelization_3.0__comparing labels just energy.pdf} }}%
%   \hfill
%   \subfloat[\centering PCA Component 24 ($-0.24\pm 0.03$)]{{\label{trueradomenergy}\includegraphics[width=0.32\linewidth]{figures/component_labeling/split_data_original_dataset_component_for_labelization_25.0__comparing labels just energy.pdf} }}%    
   
%   \caption{Energy profile of the first layer when labeling images of CIFAR10 based on their total projection on different patch-PCA components, trained with true (green line) and random (orange line) labels. Creating a correlation between the label and the PCA component causes the first layer to learn this component, depicted by a spike in the energy. Mean correlation values are in parenthesis.}\label{componentfig}
%      \vskip -0.2in
% \end{figure*}






% \begin{theorem}
% \label{thm:linearrandom}
%     As the number of patches in the training set goes to infinity, then at any iteration $t$, a linear CNN as above trained with gradient descent with learning rate $\eta$ and with random labels $y_i \in \set{ \pm 1}$, has the following energy profile w.r.t. $\lambda_i$ the i'th eigenvalue of the patch PCA:
%     \begin{equation}
%         e_i^2 = \tilde{c}\cdot \frac{\abs{1-(1-\eta \lambda_i)^t}}{\eta \sqrt{\lambda_i}} + \xi_{i}
%     \end{equation}
%     With $\tilde{c}$ a constant function of the number of training samples and $\xi_{i}$ a r.v. that depends on the initialization scheme.
% \end{theorem}
% \begin{theorem}
% \label{thm:lineartrue}
%     If the true labels are uncorrelated with the average patch then the profile of a linear model trained with true labels will be that of a linear model trained with random labels. 
% \end{theorem}


% \begin{figure*}[t!]%%
%   \vskip 0.2in
% \centerline{\includegraphics[width=\textwidth]{figures/formula_simulation/dog_vs_cat.pdf}}
%   \caption{Simulating the formula for true and random labels on the binary CIFAR10 dataset Dog vs Cat. From left to right the number of GD iterations increases (1, $10^6$, $5\times 10^6$, $10^7$ respectively) while the correlation between the profiles decreases (0.98, 0.81, 0.74, 0.67 respectively). More examples are provided in the appendix.}\label{divergence}
%      \vskip -0.2in
% \end{figure*}

==> tables.tex <==
% EXAMPLE TABLE
\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


% TABLE 1
\begin{table}[b]
\caption{Correlation between energy profiles of VGG11, trained with different random seeds (initializations), first layer widths, over various datasets, and compared with ResNet18. Standard deviation provided in cases it exceeds $0.01$.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccr}
\toprule
Dataset & Seed & Trained v & Width & VGG11 v \\
 &  & Init &  & ResNet18 \\

\midrule

CIFAR10&0.99 $\pm$ 0.004&-0.13 $\pm$ 0.18&0.98 $\pm$ 0.01&0.87 $\pm$ 0.04\\
CIFAR100&0.97 $\pm$ 0.01&-0.04 $\pm$ 0.04&0.98 $\pm$ 0.01&0.80 $\pm$ 0.02\\
CelebA&0.99 $\pm$ 0.004&-0.18 $\pm$ 0.13&0.98 $\pm$ 0.01&0.92 $\pm$ 0.02 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLE 2

\begin{table}[t]
\caption{Correlation between energy profiles of VGG11 trained with true and random labels for different datasets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Dataset & VGG (True) & VGG (Random) &  VGG (True) v \\
 &  v Init& v Init &  VGG (Random) \\

\midrule


CIFAR10&-0.13 $\pm$ 0.17&0.03 $\pm$ 0.22&\textbf{0.90 $\pm$ 0.02}\\
CIFAR100&-0.044 $\pm$ 0.04&0.14 $\pm$ 0.13&\textbf{0.91 $\pm$ 0.01}\\
CelebA&-0.18 $\pm$ 0.13&0.085 $\pm$ 0.07&\textbf{0.96 $\pm$ 0.03}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}










\begin{table}
  \caption{Correlation between energy profiles of VGG11 trained with true and random labels for different datasets as depicted in \cref{fig:vggtruerandom}. We show the average correlation (over multiple random initializations and firs layer widths) and the standard deviations. It is clear that the first layer is highly correlated when training with true and random labels.}
\begin{center}
\begin{small}
\begin{sc}
  \label{truerandomtable}
  \centering
  \begin{tabular}{lccc}
    \toprule
    % \multicolumn{4}{c}{VGG}                   \\
    % \cmidrule(r){2-5}
    Dataset     & \thead{VGG (True) \\ vs Init.} & \thead{VGG (Random) \\ vs Init.} & \thead{VGG (Random) \\ vs VGG (True)} \\
    \midrule

CIFAR10&-0.13 $\pm$ 0.17&0.03 $\pm$ 0.22&\textbf{0.90 $\pm$ 0.02}\\
CIFAR100&-0.044 $\pm$ 0.04&0.14 $\pm$ 0.13&\textbf{0.91 $\pm$ 0.01}\\
CelebA&-0.18 $\pm$ 0.13&0.085 $\pm$ 0.07&\textbf{0.96 $\pm$ 0.03}\\
    \bottomrule
  \end{tabular}
    \end{sc}
\end{small}
\end{center}
\end{table}
\begin{table}[t]
\caption{Correlation between energy profiles of VGG11 trained with true and random labels for different datasets. While they are highly correlated, they are far from initialization.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Dataset & VGG (T) & VGG (Random) &  VGG (True) v \\
 &  v Init& v Init &  VGG (Random) \\

\midrule


Cifar10&-0.13 $\pm$ 0.17&0.03 $\pm$ 0.22&\textbf{0.90 $\pm$ 0.02}\\
Cifar100&-0.04 $\pm$ 0.04&0.14 $\pm$ 0.13&\textbf{0.91 $\pm$ 0.01}\\
CelebA&-0.18 $\pm$ 0.13&0.08 $\pm$ 0.07&\textbf{0.96 $\pm$ 0.03}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
